Dependency Graph-to-String Statistical Machine Translation

We present graph-based translation models which translate source graphs into target strings. Source graphs are constructed from dependency trees with extra links so that non-syntactic phrases are connected. Inspired by phrase-based models, we first introduce a translation model which segments a graph into a sequence of disjoint subgraphs and generates a translation by combining subgraph translations left-to-right using beam search. However, similar to phrase-based models, this model is weak at phrase reordering. Therefore, we further introduce a model based on a synchronous node replacement grammar which learns recursive translation rules. We provide two implementations of the model with different restrictions so that source graphs can be parsed efficiently. Experiments on Chinese--English and German--English show that our graph-based models are significantly better than corresponding sequence- and tree-based baselines.

==> input/eg-basic.tex <==
\begin{figure}
    \centering
    \small
    
    \begin{dependency}[hide label]
    
         \begin{deptext}[column sep=0]
             he \& is \& in \& 19th \& because \& appear \& respiratory \& symptom \& by \& send \& hospital\\
             Ta \& Shi \& Yu \& ShiJiuRi \& Yin \& ChuXian \& HuXiDao \& ZhengZhuang \& Bei \& SongDao \& YiYuan\\
        \end{deptext}
        \depedge {2}{1}{}
        \depedge {10}{3}{}
        \depedge {3}{4}{}
        \depedge {10}{5}{}
        \depedge {5}{6}{}
        \depedge {8}{7}{}
        \depedge {6}{8}{}
        \depedge {10}{9}{}
        \depedge {2}{10}{}
        \depedge {10}{11}{}
        
        
        \node (rlabel) [below= 0.6cm and 0 of \wordref{2}{4}.west,anchor=east, xshift=0.2cm] {{\bf Ref}:};
        \node (plabel) [below= 0.6cm and 0 of rlabel.east,anchor=east] {{\bf HPBMT}:};
        \node (glabel) [below= 0.6cm and 0 of plabel.east,anchor=east] {{\bf SERG}:};
        \node (nlabel) [below= 0.6cm and 0 of glabel.east,anchor=east] {{\bf SNRG}:};
        
        \node [right =0 and 0.1 of rlabel.north east, anchor=north west,align=left] {he was sent to the hospital for respiratory symptoms on the 19th};
        \node [right =0 and 0.1 of plabel.north east, anchor=north west,align=left] {he is in 19 due to respiratory symptoms were sent to the hospital};
        \node [right =0 and 0.1 of glabel.north east, anchor=north west, align=left] {he was sent to hospital for respiratory symptoms on 19 september};
        \node [right =0 and 0.1 of nlabel.north east, anchor=north west, align=left] {he was sent to hospital for respiratory symptoms on 19 september};
        
    \end{dependency}
    
    \caption[Examples of translations from HPBMT, SERG, and SNRG]{Examples of translations from HPBMT, SERG, and SNRG. Compared with HPBMT, SERG and SNRG generated translations which have a better word order.}
    \label{fig:grammar:eg-basic}
\end{figure}


==> input/fig-gap.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    
    \matrix(m)[matrix of nodes, column sep=0.1cm] {
    Given:
       $s=$ & $s_1$ & $s_2$ & $s_3$ & $s_4$ & $s_5$ & $s_6$ & $s_7$ & $s_8$\\
       $\tilde{s}=$ & $s_1$ & $s_2$ & $s_3$ &  & $s_5$ &  &  & $s_8$\\
       $\tilde{s_1}=$ & $s_1$ &  & $s_3$ &  &  &  &  & \\
       $\tilde{s_2}=$ &  & $s_2$ &  &  & $s_5$ &  &  & \\
    };
    
    \end{tikzpicture}
    \caption {Illustrating the calculation of the number of gaps introduced by a rule which covers $\tilde{s}$ and has two non-terminals covering $\tilde{s_1}$ and $\tilde{s_2}$, respectively.}
    \label{fig:snrg:gap}
\end{figure}
